Knowledge-enhanced Memory Model for Emotional Support Conversation

The prevalence of mental disorders has become a significant issue, leading to the increased focus on Emotional Support Conversation as an effective supplement for mental health support. Existing methods have achieved compelling results, however, they still face three challenges: 1) variability of emotions, 2) practicality of the response, and 3) intricate strategy modeling. To address these challenges, we propose a novel knowledge-enhanced Memory mODEl for emotional suppoRt coNversation (MODERN). Specifically, we first devise a knowledge-enriched dialogue context encoding to perceive the dynamic emotion change of different periods of the conversation for coherent user state modeling and select context-related concepts from ConceptNet for practical response generation. Thereafter, we implement a novel memory-enhanced strategy modeling module to model the semantic patterns behind the strategy categories. Extensive experiments on a widely used large-scale dataset verify the superiority of our model over cutting-edge baselines.

==> parts/1_intro.tex <==
\section{Introduction}
Mental disorders are known for their high burden, with more than 50\% of adults experiencing a mental illness or disorder at some point in their lives; yet despite the high prevalence of mental illness, only one in five patients receive professional treatment\footnote{\url{https://tinyurl.com/4r8svsst}.}. 
An effective mental health intervention is to provide emotional support for people in need~\cite{green2022emotional,chang2021relationships}. 
% A considerable amount of research work has been devoted to automating mental support conversations.
As one of the most important tasks to support mental disorders, Emotional Supported Conversation (ESConv) ~\cite{DBLP:conf/acl/LiuZDSLYJH20} has attracted a lot of attention in recent years and presents a great opportunity for researchers to explore better ways to establish neural dialogue systems for mentally supported conversations. 

The ESConv takes place between a help-seeker (seeker) and a supporter in a multi-turn manner. The system expects the dialogue agent to act like the supporter role and generate responses aiming at two objects: (1) reducing the seeker's emotional distress and (2) helping the seeker overcome the challenges they face. To address this task, the agent should leverage various dialogue strategies (\eg \textit{Reflection of Feelings} and \textit{Providing Suggestions}) systematically. Besides, it also requests the agent to leverage relevant knowledge so as to raise specific and actionable suggestions for the guidance of approaching real-life difficulties.

% According to different techniques exploiting the ESConv task, previous work can be divided into two parts. 
Previous work mainly focuses on two aspects.
One trains the model to better understand contextual information (e.g., situation, seeker's emotion, and intention) in the conversations. For instance, \citeauthor{DBLP:conf/ijcai/00080XXSL22} designed a hierarchical graph network to capture both global cause and local intention. \citeauthor{DBLP:conf/acl/TuLC0W022} leveraged the power of common sense knowledge from COMET~\cite{DBLP:conf/acl/BosselutRSMCC19} to obtain a fine-grained emotion understanding.
The other trains the model to predict the dialogue strategy as accurately as possible and perform the response generation conditioned on that. For example, \citeauthor{DBLP:conf/acl/TuLC0W022} proposed to use distributed probability to select the most suitable strategy precisely. 

% Despite their great performance, we believe that these methods ignore some key points to model emotional support dialogue. One of our points of contention is the use of fine-grained dialogue strategies. Previous work employs only coarse-grained dialogue strategies, meaning only eight strategies are used/shared across all responses; however, in human dialogue, we form our response strategies based on more complex factors, e.g., seekers’ situations, emotions, and topics, etc. Simply using a strategy label to direct the generation of empathetic responses, neglecting the fact that there are more contextual meanings behind these labels is sub-optimal for generating relevant responses for a specific dialogue context.
Despite their great performance, we believe that these methods neglect two crucial points in performing the emotional support conversation.
\begin{itemize}
    \item \textbf{Neglect of concrete patterns behind the strategy categories.} 
    The concept of strategy categories is highly abstract and complex, involving various linguistic patterns \eg expression manner, wording, and phrasing. Previous work generates the response conditioned on an indicator (\ie one-hot label or latent vector) of the strategy category, ignoring its underlying semantic patterns. We argue that the strategy category is deficient in supplying the model to generate expressive and diverse responses. 
    % However, there are more semantic patterns behind the strategy category, \eg, expression manner, wording, and phrasing. As an information-increasing process, the strategy category is deficient to supply the model to generate rich and diverse responses.
    % Therefore, we form our response based on more concrete strategy features, e.g., expression manner, wording, and phrasing. Simply using a strategy label to direct the generation of supportive responses, neglecting the fact that there are more contextual meanings behind these labels, is sub-optimal for generating relevant responses.
    \item \textbf{Underutilization of multiple source knowledge.} 
    Previous studies have benefited from a single kind of commonsense knowledge. Nevertheless, the full power of multi-source knowledge, \ie concept knowledge, empathetic knowledge, and internal knowledge, remains to be harnessed. Moreover, in existing studies, knowledge only plays a role in improving dialogue context understanding. Exploring the use of multi-source knowledge to facilitate generating empathetic, informative, and supportive responses is still a blank space.  
    % How to obtain and utilize knowledge to equip the model with the ability to offer instructive problem-solving suggestions, thus helping the seekers work through challenges effectively. Moreover,
    % We argue that the model learns to generate more relevant and empathetic responses due to the need for knowledge beyond the historical context of the conversation.
\end{itemize}

% As a consequence, there are two key limitations for the ESConv task as follows,
% \begin{itemize}
%     % \item C1: How to generate responses conditioned on the fine-grained strategy category, which integrates contextual information and conversational skills.
%     \item L1: How to generate responses conditioned on the concrete strategy features instead of the abstractive category concepts.
%     \item L2: How to obtain and utilize knowledge to equip the model with the ability to offer instructive problem-solving suggestions, thus helping the seekers work through challenges effectively.
% \end{itemize}

To tackle these issues, we propose a novel \textbf{M}emory-enhanced m\textbf{OD}el \textbf{E}xploiting multi-sou\textbf{R}ce k\textbf{N}owledge for emotional support conversation, dubbed MODERN.
% \textbf{M}emory-\textbf{E}nhanced \textbf{I}nstructive for emotional support % \textbf{R}esponse generation model, dubbed MODERN, for emotional support conversation. 
As shown in Figure~\ref{fig:model}, MODERN includes three components: strategy memory-enhanced dialogue context encoding, multi-source knowledge injection, and response decoding. For modeling concrete strategy semantic patterns, we implement a memory bank that stores response representations of the different strategies separately, which serves as references when generating responses under a similar context. This allows us to implicitly ingest the complex factors behind each annotated strategy. To utilize abundant knowledge thoroughly, we acquire and integrate knowledge from three distinct sources, boosting the model to provide supportive responses with adequate empathy and information.    

Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose a novel \textbf{M}emory-enhanced m\textbf{OD}el \textbf{E}xploiting multi-sou\textbf{R}ce k\textbf{N}owledge for emotional support conversation, which adopts the memory mechanism to enrich generating expressive and diverse responses under support strategies.
    
    \item Besides widely-used commonsense knowledge, we further harness multi-source knowledge to offer empathetic and informative support effectively.

    \item Experiments on the ESConv dataset demonstrate that our model achieves state-of-the-art performance under both automatic and human evaluations.
\end{itemize}


==> parts/1_intro_leah.tex <==
\section{Introduction}
Mental disorders are known for their high burden, with more than 50\% of adults experiencing a mental illness or disorder at some point in their lives; yet despite the high prevalence of mental illness, only one in five patients receive professional treatment\footnote{\url{https://tinyurl.com/4r8svsst}.}. 
Recent studies have shown that an effective mental health intervention method is the provision of emotional support conversations~\cite{green2022emotional,chang2021relationships}. As such, Emotional Support Conversations (ESConv), as defined by ~\citet{DBLP:conf/acl/LiuZDSLYJH20}, has garnered substantial attention in recent years. They have emerged as a promising alternative strategy for mental health intervention, paving the way for the development of neural dialogue systems designed to provide support for those in need.

ESConv is designed upon ESC framework which comprises three stages: 1) Exploration, 2) Comforting, and 3) Action~\citep{DBLP:conf/acl/LiuZDSLYJH20}. These stages aim to emulate human behavior by initially identifying the seeker's problem and associated emotion, followed by selecting an appropriate support strategy to provide comfort, and ultimately offering suggestions to evoke a positive emotional response. 
Successfully implementing these stages involves effectively modeling user emotions throughout the conversations and mapping the seeker's emotions to the specific emotional concerns~\citep{DBLP:conf/aaai/ZhouHZZL18,Zwaan2012ABD,Medeiros2018UsingCF,shen-etal-2020-counseling}, thereby enabling the provision of personalized support. %相关参考文献支撑

However, to construct a comprehensive ESConv model, there are still some challenges faced by existing works, as follows: 
\begin{itemize}
    \item \textbf{\textit{Emotional Validation}}
    The act of validation is essential in making an individual feel both cared for and supported. Studies have shown how it facilitates emotional support \cite{Burleson2003, HighSteuber2014}. 
    Previous studies have employed either localized mental state models or coarse-grained, token-based emotional knowledge to enhance this form of validation \cite{Majumder2020MIMEME,DBLP:conf/emnlp/ChengLLWZLL022}.
    However, the emotional state of a conversation shifts dramatically as the conversation progresses, effectively reflecting the intensity of these emotions. A proficient ES system must be capable of accurately recognizing the fine-grained emotional states throughout the entire conversation\cite{Ding2022}.
    \item \textbf{\textit{Intricate Strategy}}
    In ESConv, strategies, text style labels, are mimicry tags utilized to guide the generation of responses. \cite{hill2009helping} However, these type of labels encapsulate a wide variety of complex and intricate linguistic features, such as persona and situations \cite{zheng-etal-2021-comae,zhong-etal-2020-towards}. While the practice of representing these strategies with a single vector or indicator has achieved great results \citet{DBLP:conf/acl/TuLC0W022}, it tends to insufficiently capture the full complexity and diversity behind the strategies.
    \item \textbf{\textit{Positive Emotional Response}}
    In the absence of explicit cues, neural dialogue systems tend to make generic responses~\cite{liu-etal-2018-towards-less}. Prior research has used knowledge to expand the scope of empathetic expressions during the generation process \cite{DBLP:conf/acl/TuLC0W022, DBLP:conf/ijcai/00080XXSL22}. However, it's remain a critical and unexplored gap in the literature concerning the effective use of knowledge to resonate with the emotional state of individuals seeking support \cite{Anneke2012}. To address the seeker's specific emotional concerns and provide personalized support, leveraging a knowledge base that links a range of emotions to real-world scenarios enables the generation of tailored responses. These responses align with the seeker's emotional state and provide meaningful assistance based on their individual needs.
\end{itemize}


To overcome these challenges, as shown in Figure~\ref{fig:model}, we introduce a novel method, \textbf{M}emory-enhanced m\textbf{OD}el \textbf{E}xploiting multi-sou\textbf{R}ce k\textbf{N}owledge for emotional support conversation, dubbed \textbf{MODERN}. The cornerstone of our model is the innovative utilization of a memory bank. We acknowledge the importance of memory in enabling humans to draw on past experiences when showing empathy, fostering a deeper connection with help-seekers' emotions and experiences. We maps strategies to historical dialogues. This way, it can detect and mimic the intricate patterns in human emotional support strategies. Consequently, our model can generate responses that are both empathetic and helpful, thereby truly encompassing the essence of emotional support conversations.

MODERN embodies a fusion of conceptual knowledge from ConceptNet~\cite{DBLP:conf/aaai/SpeerCH17} and authentic dialogues derived from ESConv data, complemented by the emotional representation facilitated by EmoRoberta \cite{9865796}. To the best of our knowledge, we are the first to detect the changing emotion in utterances to boost ESConv. This intricate blend enables the system to accurately map the shifting emotional panorama within dialogues. The system co-trains the conceptual knowledge and real-world data in synchronization with the dynamically changing emotions. This synergistic approach empowers MODERN to use knowledge effectively, resonating profoundly with the seekers' circumstances and emotional states.

We present a thorough validation and evaluation of our model, providing an in-depth analysis of the results and a comparison with other models. The extensive experiments on the ESConv dataset demonstrate that MODERN achieves state-of-the-art performance under both automatic and human evaluations. Our contributions can be summarized as follows:
\begin{itemize}
    \item We first analyze the current challenges of the ESConv task, and according to that propose a novel knowledge-enhanced Memory mODEl for emotional suppoRt coNversation, named MODERN, which can model complex dialogue strategy as well as utilize multi-source knowledge to perceive the variability of emotions and provide effective emotion support advice. 
    
    \item We propose a strategy-specific memory bank component, where a unique memory bank for each strategy is designed to model intricate strategy information and an auxiliary strategy classification task  is introduced to refine accurate strategy information in each memory bank.
    
    \item To the best of our knowledge, we are the first to detect the changing emotion in utterances to boost ESConv. Experiments on the ESConv dataset demonstrate that our model achieves state-of-the-art performance under both automatic and human evaluations.
\end{itemize}

